Video-FocalNets: Spatio-Temporal Focal Modulation for Video Action Recognition

Recent video recognition models utilize Transformer models for long-range spatio-temporal context modeling. Video transformer designs are based on self-attention that can model global context at a high computational cost. In comparison, convolutional designs for videos offer an efficient alternative but lack long-range dependency modeling. Towards achieving the best of both designs, this work proposes Video-FocalNet, an effective and efficient architecture for video recognition that models both local and global contexts. Video-FocalNet is based on a spatio-temporal focal modulation architecture that reverses the interaction and aggregation steps of self-attention for better efficiency. Further, the aggregation step and the interaction step are both implemented using efficient convolution and element-wise multiplication operations that are computationally less expensive than their self-attention counterparts on video representations. We extensively explore the design space of focal modulation-based spatio-temporal context modeling and demonstrate our parallel spatial and temporal encoding design to be the optimal choice. Video-FocalNets perform favorably well against the state-of-the-art transformer-based models for video recognition on five large-scale datasets (Kinetics-400, Kinetics-600, SS-v2, Diving-48, and ActivityNet-1.3) at a lower computational cost. Our code/models are released at https://github.com/TalalWasim/Video-FocalNets.

==> includes/figures_main/algorithm.tex <==
\begin{algorithm*}
    
    \caption{Pseudo code for Spatio-Temporal Focal Modulation.}
    \label{alg:videofocalnet}
    \scriptsize
    % \Comment{Class FocalModulate(nn.Module): init() and forward() functions}
    \Comment{Input/output shape: (B*T, H, W, C); Batchsize B; Feature map temporal length T, height H, width W, dim C}
    \Comment{Focal levels: L;  Conv kernel size at level $\ell$: k$^{\ell}$} 

    \Function{init( )}
    {
        
        \var{spatial\_pj\_in, spatial\_pj\_cxt = Linear(C, C + (L+1)), Conv2d(C, C, 1) }\;
        \var{temporal\_pj\_in, temporal\_pj\_cxt = Linear(C, C + (L+1)), Conv1d(C, C, 1) }\;
        \var{pj\_q = Linear(C, C)}\;
        \var{spatial\_hc\_layers = [Sequential(Conv2d(C, C, k$^{\ell}$, groups=C), GeLU())\forinline{for} $\ell$ in range(L)]}\;
        \var{temporal\_hc\_layers = [Sequential(Conv1d(C, C, k$^{\ell}$, groups=C), GeLU())\forinline{for} $\ell$ in range(L)]}\;
        \var{pj\_out = Sequential(Linear(C, C),  Dropout()) }\;
    }

    \Function{forward(\var{x}, \var{m=0})}
    {
        \CommentSty{query projection using $q(\cdot)$}  \;
        \var{q = \FuncCall{pj\_q}{x.reshape(B*T, H, W, C)}.\FuncCall{permute}{0, 3, 1, 2} } \;

        \CommentSty{input and gate projection using query projection using $f_{z,s}/f_{z,t}$ and $f_{g,s}/f_{g,t}$}  \;
        \var{x\_spatial = \FuncCall{spatial\_pj\_in}{x.reshape(B*T, H, W, C)}.\FuncCall{permute}{0, 3, 1, 2} } \;
        \var{x\_temporal = \FuncCall{temporal\_pj\_in}{x.reshape(B*H*W, T, C)}.\FuncCall{permute}{0, 2, 1} } \;
        \var{z\_spatial, gate\_spatial = split(x\_spatial, (C, L+1), 1)} \;
        \var{z\_temporal, gate\_temporal = split(x\_temporal, (C, L+1), 1)} \;        
        
        \For{$\ell$  in range(L)}{
            \CommentSty{~\# Eq.\eqref{eq:spt_hier_context}, spatio-temporal hierarchical contextualization}  \;
            \var{ z\_spatial = spatial\_hc\_layers[$\ell$](z\_spatial) } \;
            \var{ z\_temporal = temporal\_hc\_layers[$\ell$](z\_temporal) } \;               
            
            \CommentSty{~\# Eq.\eqref{eq:spt_gated_agg}, spatio-temporal gated aggregation}  \; 
            \var{ m\_spatial = m\_spatial +  z\_spatial * gate\_spatial[:, $\ell$:$\ell$+1] }  \; 
            \var{ m\_temporal = m\_temporal +  z\_temporal * gate\_temporal[:, $\ell$:$\ell$+1] } \; 
            
        }
        \CommentSty{\# Eq.\eqref{eq:spt_global_context}, spatio-temporal global context aggregation}  \;
        \var{m\_spatial = m\_spatial + GeLU(z\_spatial.mean(dim=(2,3))) * gate\_spatial[:,L:]} \; 
        \var{m\_temporal = m\_temporal + GeLU(z\_temporal.mean(dim=(2))) * gate\_spatial[:,L:]} \; 

        \CommentSty{\# Eq.\eqref{Eq:spt_FocalModulation}, Spatio-Temporal Focal Modulation} \; 
        \var{x = q * spatial\_pj\_cxt(m\_spatial) * temporal\_pj\_cxt(m\_temporal).reshape(B*T, H, W, C) } \;
        \Return { pj\_out( x.permute(0, 2, 3, 1) ) } \;
    }

    % \Comment{The SoftTargetCrossEntropy function}
    % \Function{SoftCE(\var{s}, \var{t})}
    % {
    %     \var{s  = softmax(\var{s}, dim=-1)} \;
    %     \var{loss = - (t * log(s)).sum(dim=-1)} \;
    %     \Return { (loss/t.sum(dim=-1)).mean() } \;
    % }
\end{algorithm*}

==> includes/figures_main/intro_graph.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkturquoise0191191}{RGB}{0,191,191}
\definecolor{darkviolet1910191}{RGB}{191,0,191}
\definecolor{goldenrod1911910}{RGB}{191,191,0}
\definecolor{green01270}{RGB}{0,127,0}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={FLOPs (G/view)},
xmajorgrids,
xmin=55, xmax=480,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Top-1 K400 Accuracy},
ymajorgrids,
ymin=78.6, ymax=83.8,
ytick style={color=black}
]
\addplot [semithick, green01270, dashed, mark=triangle, mark size=3, mark options={solid}]
table {%
88 78.8
166 80.6
282 82.7
};
\addplot [semithick, red, dashed, mark=o, mark size=3, mark options={solid}]
table {%
63 79.8
124 81.4
149 83.6
};
\addplot [semithick, darkviolet1910191, mark=pentagon, mark size=3, mark options={solid}]
table {%
390 81.5
};
\addplot [semithick, blue, mark=otimes, mark size=3, mark options={solid}]
table {%
455 81.2
};
\addplot [semithick, darkturquoise0191191, mark=square, mark size=3, mark options={solid}]
table {%
226 82.9
};
\addplot [semithick, black, mark=diamond, mark size=3, mark options={solid}]
table {%
259 83
};
\addplot [semithick, goldenrod1911910, mark=oplus, mark size=3, mark options={solid}]
table {%
399 81.8
};
\draw (axis cs:88,78.8) node[
  anchor=base west,
  text=black,
  rotate=0.0
]{\scriptsize \textbf{Video-Swin-T}~\cite{liu2021video-swin}};
\draw (axis cs:166,80.6) node[
  anchor=base west,
  text=black,
  rotate=0.0
]{\scriptsize \textbf{Video-Swin-S}~\cite{liu2021video-swin}};
\draw (axis cs:282,82.7) node[
  anchor=base west,
  text=black,
  rotate=0.0
]{\scriptsize \textbf{Video-Swin-B}~\cite{liu2021video-swin}};
\draw (axis cs:63,79.8) node[
  anchor=base west,
  text=black,
  rotate=0.0
]{\scriptsize \textbf{Video-FocalNet-T}};
\draw (axis cs:124,81.4) node[
  anchor=base west,
  text=black,
  rotate=0.0
]{\scriptsize \textbf{Video-FocalNet-S}};
\draw (axis cs:149,83.6) node[
  anchor=base west,
  text=black,
  rotate=0.0
]{\scriptsize \textbf{Video-FocalNet-B}};
\draw (axis cs:315,81.2) node[
  anchor=base west,
  text=black,
  rotate=0.0
]{\scriptsize \textbf{MoViNet-A6}~\cite{kondratyuk2021movinets}};
\draw (axis cs:365,80.9) node[
  anchor=base west,
  text=black,
  rotate=0.0
]{\scriptsize \textbf{MViTv1-B}~\cite{fan2021multiscale}};
\draw (axis cs:151,82.6) node[
  anchor=base west,
  text=black,
  rotate=0.0
]{\scriptsize \textbf{MViTv2-B}~\cite{li2022improved}};
\draw (axis cs:259,83) node[
  anchor=base west,
  text=black,
  rotate=0.0
]{\scriptsize \textbf{Uniformer-B}~\cite{li2022uniformer}};
\draw (axis cs:364,82) node[
  anchor=base west,
  text=black,
  rotate=0.0
]{\scriptsize \textbf{MTV-B}~\cite{shen2022mtv}};
\end{axis}

\end{tikzpicture}


==> includes/tables_ablation/design_choices.tex <==
\begin{table}[t]

\centering
\small
\caption{Comparison of various design choices for Video-FocalNet-S on Kinetics-400~\cite{kay2017k400} validation set.}
\setlength{\tabcolsep}{3mm}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcc}
\rowcolor{Gray}
    \toprule
    Method                                              & Top-1     & Parameters (M) \\
    \midrule
    Naive Frame Averaging                               & 74.7      & 49.4           \\
    Factorized 3D Convolution                           & 78.0      & 49.5           \\
    Factorized Encoder                                  & 79.5      & 96.8           \\
    Factorized FocalNet Block                           & 80.6      & 96.8           \\    
    \midrule
    Ours                                                & 81.4      & 88.7           \\
    \bottomrule
\end{tabular}
}
\label{tab:ablation_design_choices}
% \vspace{-.4cm}

\end{table}

==> includes/tables_ablation/fusion_type.tex <==
\begin{table}[t]

\centering
\small
\caption{Comparison of various fusion techniques for Video-FocalNet-S on Kinetics-400~\cite{kay2017k400} validation set.}
\setlength{\tabcolsep}{3mm}
\resizebox{0.7\columnwidth}{!}{
\begin{tabular}{lc}
\rowcolor{Gray}
    \toprule
    Method                            & Top-1 \\
    \midrule
    Learnable                         & 79.9  \\
    Elementwise Average               & 80.8  \\
    \midrule
    Ours (Elementwise Multiplication) & 81.4  \\
    \bottomrule
\end{tabular}
}
\label{tab:ablation_fusion_type}
% \vspace{-.4cm}

\end{table}

==> includes/tables_ablation/patch_tube_embedding.tex <==
\begin{table}[t]

\centering
\small
\caption{Comparison of use patch vs tubelet embedding for Video-FocalNet-S on Kinetics-400~\cite{kay2017k400} validation set. Note that the number of frames is adjusted accordingly to ensure that the number of tokens is the same.}
\setlength{\tabcolsep}{3mm}
\resizebox{0.7\columnwidth}{!}{
\begin{tabular}{lc}
\rowcolor{Gray}
    \toprule
    Method                      & Top-1 \\
    \midrule
    Ours + Tubelet Embedding    & 81.2  \\
    Ours + Patch Embedding      & 81.4  \\
    \bottomrule
\end{tabular}
}
\label{tab:ablation_embedding}
% \vspace{-.4cm}

\end{table}
